MIMO Multipath-based SLAM for Non-Ideal Reflective Surfaces

Multipath-based simultaneous localization and mapping (MP-SLAM) is a well established approach to obtain position information of transmitters and receivers as well as information regarding the propagation environments in future multiple input multiple output (MIMO) communication systems. Conventional methods for MP-SLAM consider specular reflections of the radio signals occurring at smooth, flat surfaces, which are modeled by virtual anchors (VAs) that are mirror images of the physical anchors (PAs), with each VA generating a single multipath component (MPC). However, non-ideal reflective surfaces (such as walls covered by shelves or cupboards) cause dispersion effects that violate the VA model and lead to multiple MPCs that are associated to a single VA. In this paper, we introduce a Bayesian particle-based sum-product algorithm (SPA) for MP-SLAM in MIMO communications systems. Our method considers non-ideal reflective surfaces by jointly estimating the parameters of individual dispersion models for each detected surface in delay and angle domain leveraging multiple-measurement-to-feature data association. We demonstrate that the proposed SLAM method can robustly and jointly estimate the positions and dispersion extents of ideal and non-ideal reflective surfaces using numerical simulation.

==> inputFiles/SPA.tex <==
%!TEX root = ../JAIF_2023_V3.tex

\section{Proposed Sum-Product Algorithm}
\label{sec:SPA}

The factor graph in Fig.~\ref{fig:FG} has cycles, therefore we have to decide on a specific order of message computation \cite{KscFreLoe:TIT2001,Loe:SMP2004_FG}. We use iterative \ac{MP} with \ac{MP} iteration $p \in \{1, \dots, P\}$ where $P$ is the maximum number of \ac{MP} iterations. 
We choose the order according to the following rules: (i) messages are only sent forward in time; (ii) for each PA, messages are updated in parallel; (iii) along an edge connecting the augmented agent state variable node and a new \ac{pva}, messages are only sent from the former to the latter; (iv) the augmented agent state variable node is only updated at \ac{MP} iteration $P$. The corresponding messages are shown in Fig.~\ref{fig:FG}. Note, that this scheduling is suboptimal since the extrinsic messages of the augmented agent state are neglected. This calculation order is solely chosen to reduce the computational demand. With these rules, the message passing equations of the \ac{spa} \cite{KscFreLoe:TIT2001} yield the following operations at each time step.

\subsection{Prediction Step}
A prediction step is performed for the augmented agent state and all legacy \acp{va} $k \in \Set{K}_{n-1}^{(j)}$. 
It has the form of
\vspace*{-1mm}
\begin{align}
\alpha(\V{x}_n) &=  \int f(\V{x}_n|\V{x}_{n-1}) b(\V{x}_{n-1}) \mathrm{d}\V{x}_{n-1} \label{eq:mp_agentPredic}\\
%
\alpha(\underline{\V{x}}^{(j)}_{k,n},\underline{r}^{(j)}_{k,n}) &=  \hspace{-2mm} \hspace{-4mm}\sum_{r^{(j)}_{k,n-1} \rmv \in \{0,1\}} \hspace{-5mm} \iint g(\underline{\V{x}}^{(j)}_{k,n},\underline{r}^{(j)}_{k,n}|\V{x}^{(j)}_{k,n-1},r^{(j)}_{k,n-1},\xn{n-1}) \nn \\
	& \hspace*{-5mm}\times b(\V{x}^{(j)}_{k,n-1},r^{(j)}_{k,n-1})  b(\V{x}_{n-1}) \mathrm{d}\V{x}^{(j)}_{k,n-1} \mathrm{d}\V{x}_{n-1} \label{eq:mp_VaPredic}
\end{align}
with $b(\V{x}_{n-1})$ and $b(\V{x}^{(j)}_{k,n-1},r^{(j)}_{k,n-1})$ denoting the beliefs of the augmented agent state and the legacy \ac{va} $k$ calculated at the previous time step, respectively. 
The summation in \eqref{eq:mp_VaPredic}, can be further written as
\begin{align}
\alpha(\underline{\V{x}}^{(j)}_{k,n},\underline{r}^{(j)}_{k,n} \rreq 1) &= p_\text{s} \rmv\rmv\rmv \iint \rmv\rmv\rmv e^{-\mumL{k}{n-1}}\rmv\rmv f(\underline{\V{x}}^{(j)}_{k,n},1|\V{x}^{(j)}_{k,n-1},1) \nn \\
	& \times b(\V{x}^{(j)}_{k,n-1},1) b(\xn{n-1}) \mathrm{d}\V{x}^{(j)}_{k,n-1} \mathrm{d}\xn{n-1}
\end{align} 
and $\alpha(\underline{\V{x}}^{(j)}_{k,n},\underline{r}^{(j)}_{k,n} \rreq 0) = \underline{\alpha}^{\text{n},(j)}_k f_\text{d}(\underline{\V{x}}^{(j)}_{k,n})$ with 
\vspace*{-1mm}
\begin{align}
	\underline{\alpha}^{\text{n},(j)}_k & \triangleq \tilde{b}_{k,n-1} + (1-p_\text{s}) \int b(\Lxn{n-1},1) \mathrm{d}\Lxn{n-1} \nn \\
	& = \tilde{b}_{k,n-1} + (1-p_\text{s})(1-\tilde{b}_{k,n-1})
\end{align}
where $\tilde{b}_{k,n-1} = \int b(\Lxn{n-1},0) \mathrm{d}\Lxn{n-1}$ approximates the probability of non-existence of legacy \ac{va} $k$. 
%For the new \acp{va}, $\alpha(\overline{\V{x}}^{(j)}_{m,n},\overline{r}^{(j)}_{m,n}) \triangleq \int f(\overline{\V{x}}^{(j)}_{m,n},\overline{r}^{(j)}_{m,n}| \xn{n-1}) b(\xn{n-1})  \mathrm{d}\xn{n-1}$ with $m \in \Set{M}^{(j)}_n$.

\subsection{Measurement Evaluation}
The messages $\varepsilon^{[p]}(\al)$ sent from factor nodes $q(\x,\underline{\V{y}}^{(j)}_{k,n},\al,\V{z}^{(j)}_{l,n})$ to variable nodes $\al$ at \ac{MP} iteration $p$ with $k \in \{1,\dots,K_{n-1}^{(j)}\}$ and $l \in \{1,\dots,M_n^{(j)}\}$ are defined as
\begin{align}
	\varepsilon^{[p]}(\al) =&   \iint \tilde{\beta}^{[p]}_{kl}(\V{x}_n) \alpha^{[p]}_l(\underline{\V{y}}^{(j)}_{k,n}) \nn \\
	& \times q(\x,\underline{\V{y}}^{(j)}_{k,n},\al,\V{z}^{(j)}_{l,n}) \mathrm{d}\V{x}_n \mathrm{d}\underline{\V{y}}^{(j)}_{k,n}.
	\label{eq:message_epsilon1}
\end{align}
The messages from factor nodes $u(\x,\overline{\V{y}}^{(j)}_{k,n},\an{k}{l},\V{z}^{(j)}_{l,n})$ to variable nodes $\an{k}{l}$ where $k \in\{1,\dots,M_n^{(j)}\}$ and $l \in \{1,\dots,M_n^{(j)} \}\backslash k $, are given as
\begin{align}
	\varepsilon^{[p]}(\an{k}{l}) =&   \iint \tilde{\beta}^{[p]}_{kl}(\V{x}_n) \alpha^{[p]}_l(\overline{\V{y}}^{(j)}_{k,n}) \nn \\
	& \times u(\V{x}_n,\overline{\V{y}}^{(j)}_{k,n},\an{k}{l},\V{z}^{(j)}_{l,n}) \mathrm{d}\V{x}_n \mathrm{d}\overline{\V{y}}^{(j)}_{k,n}
	\label{eq:message_epsilon2}
\end{align}
and the messages from factor nodes $v(\x,\overline{\V{y}}^{(j)}_{m,n},\overline{a}^{(j)}_{mm,n},\V{z}^{(j)}_{m,n})$ to variable nodes $\overline{a}^{(j)}_{mm,n}$, $m \in\{1,\dots,M_n^{(j)}\}$, are given as
\begin{align}
	\varepsilon^{[p]}(\overline{a}^{(j)}_{mm,n}) =&   \iint \tilde{\beta}^{[p]}_{mm}(\V{x}_n) \alpha^{[p]}_m(\overline{\V{y}}^{(j)}_{m,n}) \nn \\
	& \times v(\V{x}_n,\overline{\V{y}}^{(j)}_{m,n},\overline{a}^{(j)}_{mm,n},\V{z}^{(j)}_{m,n}) \mathrm{d}\V{x}_n \mathrm{d}\overline{\V{y}}^{(j)}_{m,n}.
	\label{eq:message_epsilon3}
\end{align}
Note that $\alpha^{[p=1]}_l(\underline{\V{y}}^{(j)}_{k,n}) \triangleq \alpha(\underline{\V{x}}^{(j)}_{k,n},\underline{r}^{(j)}_{k,n})$ and $\alpha^{[p=1]}_l(\overline{\V{y}}^{(j)}_{k,n}) \triangleq 1$. 
For $p>1$, $\alpha^{[p]}_l({\V{y}}^{(j)}_{k,n})$ is calculated according to Section~\ref{sec:ExtrInfo}. 
The message $\tilde{\beta}^{[p]}_{kl}(\V{x}_n)$ will be defined in Section~\ref{sec:MP_updateAgent}.
Using \eqref{eq:message_epsilon1}, $\varepsilon^{[p]}(\al)$ is further investigated. 
For the messages containing information about legacy \acp{va}, it results in
\begin{align}
	\varepsilon^{[p]}(\underline{a}^{(j)}_{kl,n} \rreq 1) =& \iint \tilde{\beta}^{[p]}_{kl}(\V{x}_n) \alpha^{[p]}_l(\underline{\V{x}}^{(j)}_{k,n},\underline{r}^{(j)}_{k,n} \rreq 1)  \nn \\
	& \times \frac{\mu_\text{m}\big(\V{x}_n,\underline{\V{x}}^{(j)}_{k,n} \big) f(\V{z}^{(j)}_{l,n}|\V{x}_n,\underline{\V{x}}^{(j)}_{k,n})}{\mu_\text{fa} f_\text{fa}(\V{z}^{(j)}_{l,n})} \mathrm{d}\underline{\V{x}}^{(j)}_{k,n} \mathrm{d}\V{x}_n \nonumber \\
	\varepsilon^{[p]}(\underline{a}^{(j)}_{kl,n} \rreq 0) =& \iint  \tilde{\beta}^{[p]}_{kl}(\V{x}_n) \Big( \alpha^{[p]}_l(\underline{\V{x}}^{(j)}_{k,n},\underline{r}^{(j)}_{k,n} \rreq 1)  \nn \\
	&   \hspace*{4mm} + \alpha^{[p]}_l(\underline{\V{x}}^{(j)}_{k,n},\underline{r}^{(j)}_{k,n} \rreq 0)\Big) \mathrm{d}\underline{\V{x}}^{(j)}_{k,n} \mathrm{d}\V{x}_n.
	\label{eq:epsilon_legacy}
\end{align}
This can be further simplify by dividing both messages by $\varepsilon^{[p]}(\underline{a}^{(j)}_{kl,n} = 0)$. 
With an abuse of notation, it results in $\varepsilon^{[p]}(\underline{a}^{(j)}_{kl,n} \rreq 0) = 1$. 

The messages $\varepsilon^{[p]}(\overline{a}^{(j)}_{kl,n})$ can be obtained similarly by using \eqref{eq:message_epsilon2} and \eqref{eq:message_epsilon3}, yielding
\begin{align}
&\varepsilon^{[p]}(\overline{a}^{(j)}_{kl,n} \rreq 1) = \iint \tilde{\beta}^{[p]}_{kl}(\V{x}_n) \alpha^{[p]}_l(\overline{\V{x}}^{(j)}_{k,n},\overline{r}^{(j)}_{k,n} \rreq 1) \nn \\
	& \hspace{2mm}  \times \frac{f(\Nx{k}|\x) \mumN{k}{n} f(\V{z}^{(j)}_{l,n}|\V{x}_n,\overline{\V{x}}^{(j)}_{k,n})}{\mu_\text{fa} f_\text{fa}(\V{z}^{(j)}_{l,n})} \mathrm{d}\overline{\V{x}}^{(j)}_{k,n} \mathrm{d}\V{x}_n \\
%
&\varepsilon^{[p]}(\overline{a}^{(j)}_{kl,n} \rreq 0) = \iint \tilde{\beta}^{[p]}_{kl}(\V{x}_n) \Big( \alpha^{[p]}_l(\overline{\V{x}}^{(j)}_{k,n},\overline{r}^{(j)}_{k,n} \rreq 1)  \nn \\
	& \hspace{23mm}  + \alpha^{[p]}_l(\overline{\V{x}}^{(j)}_{k,n},\overline{r}^{(j)}_{k,n} \rreq 0)  \Big) \mathrm{d}\overline{\V{x}}^{(j)}_{k,n} \mathrm{d}\V{x}_n
\end{align}
\begin{align}
&\varepsilon^{[p]}(\overline{a}^{(j)}_{mm,n} \rreq 1)  =  \iint \tilde{\beta}^{[p]}_{mm}(\V{x}_n) \alpha^{[p]}_m(\overline{\V{x}}^{(j)}_{m,n},\overline{r}^{(j)}_{m,n} \rreq 1)  \nn \\
 &\hspace{0mm}\times \frac{f(\Nx{m}|\x) \mu_\text{m}\big(\V{x}_n,\overline{\V{x}}^{(j)}_{m,n} \big) f(\V{z}^{(j)}_{m,n}|\V{x}_n,\overline{\V{x}}^{(j)}_{m,n})}{\mu_\text{fa} f_\text{fa}(\V{z}^{(j)}_{m,n})} \mathrm{d}\overline{\V{x}}^{(j)}_{m,n} \mathrm{d}\V{x}_n\\
	%
& \varepsilon^{[p]}(\overline{a}^{(j)}_{mm,n} \rreq 0) \rmv\rmv=\rmv\rmv\rmv\rmv\rmv  \nn \\
&\hspace{10mm} \iint \rmv\rmv \tilde{\beta}^{[p]}_{mm}(\V{x}_n) \alpha^{[p]}_m(\overline{\V{x}}^{(j)}_{m,n},\overline{r}^{(j)}_{m,n} \rreq 0)  \mathrm{d}\overline{\V{x}}^{(j)}_{m,n} \mathrm{d}\V{x}_n
\end{align}
The expressions can be simplified by dividing all messages by $\varepsilon(\overline{a}^{(j)}_{kl,n} = 0)$. With an abuse of notation, it results in $\varepsilon(\overline{a}^{(j)}_{kl,n} = 0) = 1$ and
\begin{align}
&\varepsilon^{[p]}(\overline{a}^{(j)}_{mm,n} \rreq 0)   \nn \\
&\hspace*{0mm}	=\frac{\iint  \tilde{\beta}^{[p]}_{mm}(\V{x}_n) \alpha^{[p]}_m(\overline{\V{x}}^{(j)}_{m,n}, 0) \mathrm{d}\overline{\V{x}}^{(j)}_{m,n} \mathrm{d}\V{x}_n}{\iint  \tilde{\beta}^{[p]}_{mm}(\V{x}_n) \Big(\alpha^{[p]}_m(\overline{\V{x}}^{(j)}_{m,n},1) + \alpha^{[p]}_m(\overline{\V{x}}^{(j)}_{m,n}, 0)\Big)\mathrm{d}\overline{\V{x}}^{(j)}_{m,n} \mathrm{d}\V{x}_n}
\end{align} 
%For $\varepsilon^{[p]}(\overline{a}^{(j)}_{mm,n})$, the messages differ, which leads to 
%\begin{align}
%\hspace*{-2mm}&\varepsilon^{[p]}(\overline{a}^{(j)}_{mm,n} \rreq 1)  \nn \\
%&\hspace*{0mm} = \frac{\iint \alpha^{[p]}_m(\overline{\V{x}}^{(j)}_{m,n}, 1) \frac{\mu_\text{m}\big(\V{x}_n,\overline{\V{x}}^{(j)}_{m,n} \big) f(\V{z}^{(j)}_{m,n}|\V{x},\overline{\V{x}}^{(j)}_{m,n})}{\mu_\text{fa} f_\text{fa}(\V{z}^{(j)}_{m,n})} \mathrm{d}\overline{\V{x}}^{(j)}_{m,n} \mathrm{d}\V{x}_n}{\iint \alpha^{[p]}_m(\overline{\V{x}}^{(j)}_{m,n}, 1) + \alpha^{[p]}_m(\overline{\V{x}}^{(j)}_{m,n}, 0)\mathrm{d}\overline{\V{x}}^{(j)}_{m,n} \mathrm{d}\V{x}_n}\\
%	%
%&\varepsilon^{[p]}(\overline{a}^{(j)}_{mm,n} \rreq 0)   \nn \\
%&\hspace*{0mm}	= 1- \frac{\iint \alpha^{[p]}_m(\overline{\V{x}}^{(j)}_{m,n}, 1) \mathrm{d}\overline{\V{x}}^{(j)}_{m,n} \mathrm{d}\V{x}_n}{\iint \alpha^{[p]}_m(\overline{\V{x}}^{(j)}_{m,n},1) + \alpha^{[p]}_m(\overline{\V{x}}^{(j)}_{m,n}, 0)\mathrm{d}\overline{\V{x}}^{(j)}_{m,n} \mathrm{d}\V{x}_n}
%\end{align}

\subsection{Data Association}

The messages $\varphi^{[p]}_{kl}(b^{(j)}_{l,n})$ sent from factor node $\Psi({a}^{(j)}_{kl},b^{(j)}_l)$ to variable node $b^{(j)}_{l,n}$ and the message $\nu^{[p]}_{kl}(a^{(j)}_{kl,n})$ sent from factor node  $\Psi({a}^{(j)}_{kl},b^{(j)}_l)$ to variable node $a^{(j)}_{kl,n}$ are calculated using the measurement evaluation messages in  \eqref{eq:message_epsilon1}, \eqref{eq:message_epsilon2} and \eqref{eq:message_epsilon3}. Details can be found in Appendix~\ref{sec:DA}.

\subsection{Measurement update for \acp{pva}}
Next, we determine the messages sent from factor node $q(\V{x}_n,\underline{\V{y}}^{(j)}_{k,n},\underline{a}^{(j)}_{kl},\V{z}^{(j)}_{l,n})$ to variable node $\underline{\V{y}}^{(j)}_{k,n}$ as
\vspace*{-1mm}
\begin{align}
\gamma^{[p]}_l(\underline{\V{y}}^{(j)}_{k,n}) &= \hspace{-3mm} \sum_{\underline{a}^{(j)}_{kl,n} \in \{0,1\}} \hspace{-1mm}  \int  q(\V{x}_n,\underline{\V{x}}^{(j)}_{k,n},\underline{r}^{(j)}_{k,n},\underline{a}^{(j)}_{kl,n},\V{z}^{(j)}_{l,n})\nn\\
&\hspace*{4mm}\times \underline{\nu}^{[p]}_{kl}(\underline{a}^{(j)}_{kl,n}) \mathrm{d}\V{x}_n\\[-7mm]\nn
\end{align}
which results after marginalizing $\underline{a}^{(j)}_{kl,n}$ in 
\begin{align}
\gamma^{[p]}_l(\underline{\V{x}}^{(j)}_{k,n},\underline{r}^{(j)}_k \rreq 1) &= \int q(\V{x}_n,\underline{\V{x}}^{(j)}_{k,n},1,1,\V{z}^{(j)}_{l,n})\underline{\nu}^{[p]}_{kl}(1) \mathrm{d}\V{x}_n \nn \\
&\hspace*{4mm} + \underline{\nu}^{[p]}_{kl}(0) \\
%
\gamma^{[p]}_l(\underline{\V{x}}^{(j)}_{k,n},\underline{r}^{(j)}_k \rreq 0) &=  \underline{\nu}^{[p]}_{kl}(0)\ist.
\end{align}
%
The messages from factor node $u(\V{x}_n,\overline{\V{y}}^{(j)}_{k,n},\overline{a}^{(j)}_{kl},\V{z}^{(j)}_{l,n})$ to variable node $\overline{\V{y}}^{(j)}_{k,n}$ are given as
\begin{align}
\gamma^{[p]}_l(\overline{\V{y}}^{(j)}_{k,n}) &= \hspace{-3mm} \sum_{\overline{a}^{(j)}_{kl,n} \in \{0,1\}} \hspace{-1mm}  \int  u(\V{x}_n,\overline{\V{x}}^{(j)}_{k,n},\overline{r}^{(j)}_{k,n},\overline{a}^{(j)}_{kl,n},\V{z}^{(j)}_{l,n})\nn\\
&\hspace*{4mm}\times \overline{\nu}^{[p]}_{kl}(\overline{a}^{(j)}_{kl,n}) \mathrm{d}\V{x}_n\\[-7mm]\nn
\end{align}
which results after marginalizing $\overline{a}^{(j)}_{kl,n}$ in 
\begin{align}
\gamma^{[p]}_l(\overline{\V{x}}^{(j)}_{k,n},\overline{r}^{(j)}_k \rreq 1) &= \int u(\V{x}_n,\overline{\V{x}}^{(j)}_{k,n},1,1,\V{z}^{(j)}_{l,n})\overline{\nu}^{[p]}_{kl}(1) \mathrm{d}\V{x}_n \nn \\
&\hspace*{4mm} + \overline{\nu}^{[p]}_{kl}(0) \\
%
\gamma^{[p]}_l(\overline{\V{x}}^{(j)}_{k,n},\overline{r}^{(j)}_k \rreq 0) &=  \overline{\nu}^{[p]}_{kl}(0)\ist.
\end{align}
%
%
The message from factor node $v(\V{x}_n,\overline{\V{y}}^{(j)}_{m,n},\overline{a}^{(j)}_{mm},\V{z}^{(j)}_{m,n})$ to variable node $\overline{\V{y}}^{(j)}_{m,n}$ is given by
\begin{align}
\gamma^{[p]}_m(\overline{\V{y}}^{(j)}_{m,n}) &= \sum_{\overline{a}^{(j)}_{mm,n} \in \{0,1\}} \hspace{-1mm}  \int \rrmv v(\V{x}_n,\overline{\V{y}}^{(j)}_{m,n},\overline{a}^{(j)}_{mm,n},\V{z}^{(j)}_{m,n})\nn \\
& \hspace*{10mm}\times \overline{\nu}^{[p]}_{mm}(\overline{a}^{(j)}_{mm,n}) \mathrm{d}\V{x}_n
\end{align}
resulting in 
\begin{align}
\hspace*{-2mm}\gamma^{[p]}_m(\overline{\V{x}}^{(j)}_{m,n}, 1) &= \int v(\V{x}_n,\overline{\V{x}}^{(j)}_{m,n},1,1,\V{z}^{(j)}_{m,n})\overline{\nu}^{[p]}_{mm}(1)\mathrm{d}\V{x}_n \\
%
\hspace*{-2mm}\gamma^{[p]}_m(\overline{\V{x}}^{(j)}_{m,n}, 0) &=  \overline{\nu}^{[p]}_{mm}(0)\ist.
\end{align}
%
The messages are initialized with $\gamma^{[p=1]}_\ell(\V{y}^{(j)}_{k,n}) = 1$.

\subsection{Extrinsic Information}
\label{sec:ExtrInfo}
For each legacy \ac{va}, the messages sent from variable node $\underline{\V{y}}^{(j)}_{k,n}$ to factor nodes $q( \V{x}_n, \underline{\V{y}}^{(j)}_{k,n}, \underline{a}^{(j)}_{kl,n}; \V{z}^{(j)}_{l,n} )$ with $k \in \Set{K}^{(j)}_{n-1}$, $l \in \Set{M}^{(j)}_{n}$ at \ac{MP} iteration $p+1$ are defined as
\vspace*{-1.5mm}
\begin{align}
	\alpha^{[p+1]}_l(\underline{\V{y}}^{(j)}_{k,n}) & = \alpha(\underline{\V{y}}^{(j)}_{k,n}) \prod_{\substack{\ell = 1 \\ \ell \neq l}}^{M_n^{(j)}} \gamma^{[p]}_\ell(\underline{\V{y}}^{(j)}_{k,n})\ist.\\[-7.5mm]\nn
\end{align}
For new \acp{va}, a similar expression can be obtained for the messages from variable node  $\overline{\V{y}}^{(j)}_{m,n}$ to factor nodes $u( \V{x}_n, \overline{\V{y}}^{(j)}_{m,n}, \overline{a}^{(j)}_{ml,n}; \V{z}^{(j)}_{l,n} )$ and factor node $v(\V{x}_n, \overline{\V{y}}^{(j)}_{m,n}, \overline{a}^{(j)}_{mm,n}; \V{z}^{(j)}_{m,n} )$, i.e.,
\vspace*{-1mm}
\begin{align}
\alpha^{[p+1]}_l(\overline{\V{y}}^{(j)}_{m,n}) & = \alpha(\overline{\V{y}}^{(j)}_{m,n}) \prod_{\substack{\ell = 1 \\ \ell \neq l}}^m \gamma^{[p]}_\ell(\overline{\V{y}}^{(j)}_{m,n})\ist.\\[-7.5mm]\nn
\end{align}

\subsection{Measurement update for augmented agent state}
\label{sec:MP_updateAgent}
Due to the proposed scheduling, the augmented agent state is only updated by messages of legacy PVAs and only at the end of the iterative message passing. 
This results in 
\begin{align}
\tilde{\beta}^{[p]}_{kl}(\V{x}_n) &= \alpha(\V{x}_n) \label{eq:betaTilde}\\
\beta^{[p](j)}_{kl}(\V{x}_n) &= \sum_{\underline{a}^{(j)}_{kl,n} \in \{0,1\}} \sum_{\underline{r}^{(j)}_{k,n} \in \{0,1\}} \int \alpha_l^{[p]}(\underline{\V{x}}^{(j)}_{k,n},\underline{r}^{(j)}_{k,n}) \nn \\
& \hspace{-7mm} \times q(\V{x}_n,\underline{\V{x}}^{(j)}_{k,n},\underline{r}^{(j)}_{k,n},\underline{a}^{(j)}_{kl,n},\V{z}^{(j)}_{l,n})\underline{\nu}^{[p]}_{kl}(\underline{a}^{(j)}_{kl,n}) \mathrm{d}\underline{\V{x}}^{(j)}_{k,n}
\end{align}
which can be further simplified to 
\begin{align}
\beta^{[p](j)}_{kl}(\V{x}_n) &= \int \alpha_l^{[p]}(\V{x}^{(j)}_{k,n},1) \Big( q(\V{x}_n,\underline{\V{x}}^{(j)}_{k,n},1,1,\V{z}^{(j)}_{l,n})\underline{\nu}^{[p]}_{kl}(1)   \nn \\
&\hspace*{3mm} + \underline{\nu}^{[p]}_{kl}(0) \Big)\mathrm{d}\underline{\V{x}}^{(j)}_{k,n} +\underline{\alpha}_k^{\text{n},(j)} \underline{\nu}^{[p]}_{kl}(0).
\end{align}

\subsection{Belief calculation}
Once all messages are available and $p=P$, the beliefs approximating the desired marginal posterior \ac{pdf}s are obtained. 
The belief for the augmented agent state is given, up to a normalization factor, by 
\begin{align}
b(\V{x}_n) \propto  \alpha(\V{x}_n)  \prod_{j = 1}^J \ \prod_{k = 1}^{K_{n-1}^{(j)}} \ \prod_{m = 1}^{M_{n}^{(j)}} \beta^{[P](j)}_{km}(\V{x}_n)
\end{align}
where we only use messages from legacy \acp{va}.
This belief (after normalization) provides an approximation of the marginal posterior \ac{pdf} $f(\V{x}_n |\V{z}_{1:n})$, and it is used instead of $f(\V{x}_n |\V{z}_{1:n})$ in \eqref{eq:MMSEagent}. Furthermore, the beliefs of the legacy \acp{va} $b(\underline{\V{y}}^{(j)}_k)$ and new \acp{va} $b(\overline{\V{y}}^{(j)}_k)$ are given as
\vspace*{-2mm}
\begin{align}
b(\underline{\V{y}}^{(j)}_{k,n}) &\propto \alpha(\underline{\V{y}}^{(j)}_{k,n}) \prod_{l = 1}^{M_{n}^{(j)}} \gamma^{[P]}_l(\underline{\V{y}}^{(j)}_{k,n}) \\
%
b(\overline{\V{y}}^{(j)}_{m,n}) &\propto \alpha(\overline{\V{y}}^{(j)}_{m,n}) \prod_{l = 1}^m \gamma^{[P]}_l(\overline{\V{y}}^{(j)}_{m,n})\\[-7mm]\nn
\end{align}
A computationally feasible approximate calculation of the various messages and beliefs can be based on the sequential Monte Carlo (particle-based) implementation approach introduced in \cite{MeyHliHla:TSPIN2016,MeyerProc2018, LiLeiVenTuf:TWC2022}.





==> inputFiles/Wgroup-Teaching-Preamble.tex <==
% Greek lowercase letters, sans serif font - by Guido

%\@ifpackageloaded{<name>}{<true>}{<false>}
\usepackage{bm}

%% =========== Euler ==========
%\DeclareMathAlphabet{\matheur}{U}{eur}{m}{n}
%\SetMathAlphabet{\matheur}{bold}{U}{eur}{b}{n}
%\DeclareRobustCommand{\msf}[1]{%
%  \ifcat\noexpand#1\relax\msfgreek{#1}\else\matheur{#1}\fi%for math sans serif (Euler)
%}
%% =========================
%
%% ==== Computer Modern Sans Serif ====
\DeclareMathAlphabet{\mathsfbr}{OT1}{cmss}{m}{n}%for math sans serif (cmss)
\SetMathAlphabet{\mathsfbr}{bold}{OT1}{cmss}{bx}{n}%for math sans serif (cmss)
\DeclareRobustCommand{\msf}[1]{%
  \ifcat\noexpand#1\relax\msfgreek{#1}\else\mathsfbr{#1}\fi%for math sans serif (cmss)
}
%% =========================

% ==== Computer Modern Bright ====
%% Part 1: This is necessary to fix a bug in the .fd file of the font!!!
%\DeclareFontFamily{OT1}{cmbr}{\hyphenchar\font45 }
%\DeclareFontShape{OT1}{cmbr}{m}{n}{%
%  <-9>cmbr8
%  <9-10>cmbr9
%  <10-17>cmbr10
%  <17->cmbr17
%}{}
%\DeclareFontShape{OT1}{cmbr}{m}{sl}{%
%  <-9>cmbrsl8
%  <9-10>cmbrsl9
%  <10-17>cmbrsl10
%  <17->cmbrsl17
%}{}
%\DeclareFontShape{OT1}{cmbr}{m}{it}{%
%  <->ssub*cmbr/m/sl
%}{}
%\DeclareFontShape{OT1}{cmbr}{b}{n}{%
%  <->ssub*cmbr/bx/n
%}{}
%\DeclareFontShape{OT1}{cmbr}{bx}{n}{%
%  <->cmbrbx10
%}{}
%% Part 2
%\DeclareMathAlphabet{\mathsfbr}{OT1}{cmbr}{m}{n}%for math sans serif bright (cmbr)
%\SetMathAlphabet{\mathsfbr}{bold}{OT1}{cmbr}{b}{n}%for math sans serif bright (cmbr)
%\DeclareRobustCommand{\msf}[1]{%
%  \ifcat\noexpand#1\relax\msfgreek{#1}\else\mathsfbr{#1}\fi%for math sans serif bright (cmbr)
%}
%% =========================

\makeatletter
\newcommand{\msfgreek}[1]{\csname s\expandafter\@gobble\string#1\endcsname}
\makeatother

% Sans serif greek
\DeclareFontEncoding{LGR}{}{} % or load \usepackage{textgreek}
\DeclareSymbolFont{sfgreek}{LGR}{cmss}{m}{n}
\SetSymbolFont{sfgreek}{bold}{LGR}{cmss}{bx}{n}
\DeclareMathSymbol{\salpha}{\mathord}{sfgreek}{`a}
\DeclareMathSymbol{\sbeta}{\mathord}{sfgreek}{`b}
\DeclareMathSymbol{\sgamma}{\mathord}{sfgreek}{`g}
\DeclareMathSymbol{\sdelta}{\mathord}{sfgreek}{`d}
\DeclareMathSymbol{\sepsilon}{\mathord}{sfgreek}{`e}
\DeclareMathSymbol{\szeta}{\mathord}{sfgreek}{`z}
\DeclareMathSymbol{\seta}{\mathord}{sfgreek}{`h}
\DeclareMathSymbol{\stheta}{\mathord}{sfgreek}{`j}
\DeclareMathSymbol{\siota}{\mathord}{sfgreek}{`i}
\DeclareMathSymbol{\skappa}{\mathord}{sfgreek}{`k}
\DeclareMathSymbol{\slambda}{\mathord}{sfgreek}{`l}
\DeclareMathSymbol{\smu}{\mathord}{sfgreek}{`m}
\DeclareMathSymbol{\snu}{\mathord}{sfgreek}{`n}
\DeclareMathSymbol{\sxi}{\mathord}{sfgreek}{`x}
\DeclareMathSymbol{\somicron}{\mathord}{sfgreek}{`o}
\DeclareMathSymbol{\spi}{\mathord}{sfgreek}{`p}
\DeclareMathSymbol{\srho}{\mathord}{sfgreek}{`r}
\DeclareMathSymbol{\ssigma}{\mathord}{sfgreek}{`s}
\DeclareMathSymbol{\stau}{\mathord}{sfgreek}{`t}
\DeclareMathSymbol{\supsilon}{\mathord}{sfgreek}{`u}
\DeclareMathSymbol{\sphi}{\mathord}{sfgreek}{`f}
\DeclareMathSymbol{\schi}{\mathord}{sfgreek}{`q}
\DeclareMathSymbol{\spsi}{\mathord}{sfgreek}{`y}
\DeclareMathSymbol{\somega}{\mathord}{sfgreek}{`w}
\let\svarepsilon\sepsilon
\let\svartheta\stheta
\let\svarpi\spi
\let\svarrho\srho
\DeclareMathSymbol{\svarsigma}{\mathord}{sfgreek}{`c}
\let\svarphi\sphi
\DeclareMathSymbol{\sGamma}{\mathalpha}{sfgreek}{`G}
\DeclareMathSymbol{\sDelta}{\mathalpha}{sfgreek}{`D}
\DeclareMathSymbol{\sTheta}{\mathalpha}{sfgreek}{`J}
\DeclareMathSymbol{\sLambda}{\mathalpha}{sfgreek}{`L}
\DeclareMathSymbol{\sXi}{\mathalpha}{sfgreek}{`X}
\DeclareMathSymbol{\sPi}{\mathalpha}{sfgreek}{`P}
\DeclareMathSymbol{\sSigma}{\mathalpha}{sfgreek}{`S}
\DeclareMathSymbol{\sUpsilon}{\mathalpha}{sfgreek}{`U}
\DeclareMathSymbol{\sPhi}{\mathalpha}{sfgreek}{`F}
\DeclareMathSymbol{\sPsi}{\mathalpha}{sfgreek}{`Y}
\DeclareMathSymbol{\sOmega}{\mathalpha}{sfgreek}{`W}

\DeclareRobustCommand{\mcal}[1]{%
  \ifcat\noexpand#1\relax\mathnormal{#1}\else\cal{#1}\fi
}
\DeclareRobustCommand{\BM}[1]{%
  \ifcat\noexpand#1\relax\bm{\boldUppercaseItalicGreek{#1}}\else\bm{#1}\fi
}
\makeatletter
\newcommand{\boldUppercaseItalicGreek}[1]{\csname var\expandafter\@gobble\string#1\endcsname}
\makeatother
%-------------------------
% Math symbol
%-------------------------
%\newcommand{\rv}[1]{\MakeLowercase{\msf{#1}}}  
%\newcommand{\RV}[1]{\bm{\MakeLowercase{\msf{#1}}}}
%\newcommand{\RM}[1]{\bm{\MakeUppercase{\msf{#1}}}}
%\newcommand{\RS}[1]{\MakeUppercase{\msf{#1}}}
\newcommand{\rv}[1]{\msf{#1}}
\newcommand{\RV}[1]{\bm{\msf{#1}}}
\newcommand{\RM}[1]{\bm{\msf{#1}}}
\newcommand{\RS}[1]{\msf{#1}}

\newcommand{\V}[1]{\bm{#1}}
\newcommand{\M}[1]{\BM{#1}}
\newcommand{\Set}[1]{{\mcal{#1}}}


==> inputFiles/acronyms_unsorted.tex <==
% Acronym definitions: SORT ALPHABETICALLY!!!! life's too short: in bash 'sort acronyms.tex > acronyms_sorted.tex'

\acrodef{pa}[PA]{physical anchor}
\acrodef{mimo}[MIMO]{multiple input multiple output}
\acrodef{awgn}[AWGN]{additive white Gaussian noise}
\acrodef{bw}[BW]{bandwidth}
\acrodef{blt}[BLT]{bluetooth}
\acrodef{cdf}[CDF]{cumulative distribution function}
\acrodef{crlb}[CRLB]{Cram\'er-Rao lower bound}
\acrodef{dmc}[DMC]{dense multipath component}
\acrodef{dut}[DUT]{device under test}
\acrodef{eirp}[EIRP]{equivalent isotropic radiated power}
\acrodefplural{esl}[ESLs]{electronic shelf labels}
\acrodef{los}[LOS]{line-of-sight}
\acrodef{mf}[MF]{matched filter}
\acrodef{ml}[ML]{maximum likelihood}
\acrodef{mpc}[MPC]{multipath component}
\acrodef{nlos}[NLOS]{non-\ac{los}}
\acrodef{pcb}[PCB]{printed circuit board}
\acrodef{pdf}[PDF]{probability density function}
\acrodef{reb}[REB]{ranging error bound}
\acrodef{rss}[RSS]{received signal strength}
\acrodef{smc}[SMC]{specular multipath component}
\acrodef{snr}[SNR]{signal-to-noise-ratio}
\acrodef{sinr}[SINR]{signal-to-interference-plus-noise-ratio}
\acrodef{tdoa}[TDOA]{time difference of arrival}
\acrodef{tka}[TKA]{trusted keyless access}
\acrodef{toa}[TOA]{time-of-arrival}
\acrodef{aoa}[AOA]{angle-of-arrival}
\acrodef{uwb}[UWB]{ultra wide band}
\acrodef{mie}[MIE]{method of interval estimation}
\acrodef{mc}[MC]{Monte Carlo}
\acrodef{mse}[MSE]{mean squared error}
\acrodef{ci}[CI]{confidence interval}
\acrodef{cl}[CL]{confidence level}
\acrodef{pdp}[PDP]{power delay profile}
\acrodef{dps}[DPS]{delay power spectrum}
\acrodef{dm}[DM]{dense multipath}
\acrodef{nlike}[NLIKE]{normalized likelihood}
\acrodef{zzb}[ZZB]{Ziv-Zakai bound}
\acrodef{ut}[UT]{unscented transform}
\acrodef{glrt}[GLRT]{generalized likelihood ratio test}
\acrodef{mse}[MSE]{mean squared error}
\acrodef{rmse}[RMSE]{root mean squared error}
\acrodef{nnlike}[NNLIKE]{normalized noise-free likelihood}
\acrodef{stdv}[STDV]{standard deviation}
\acrodef{rv}[RV]{random variable}
\acrodef{bp}[BP]{belief propagation}
\acrodef{pda}[PDA]{probabilistic data association}
\acrodef{mp}[MP]{multipath}
\acrodef{pmf}[PMF]{probability mass function}
\acrodef{pdaf}[PDAF]{probabilistic data association filter}
\acrodef{pdaai}[AIPDA]{amplitude-information \ac{pda}}
\acrodef{olos}[OLOS]{obstructed \ac{los}}
\acrodef{spa}[SPA]{sum-product algorithm}
\acrodef{mmse}[MMSE]{minimum mean-square error}
\acrodef{lhf}[LHF]{likelihood function}
\acrodef{fa}[FA]{false alarm}
\acrodef{ceda}[CEDA]{channel estimation and detection algorithm}
\acrodef{pcrlb}[PCRLB]{posterior Cram\'er-Rao lower bound}
\acrodef{slam}[SLAM]{simultaneous localization and mapping}
% \acrodef{mpslam}[MP-SLAM]{multipath-based SLAM}
\acrodef{va}[VA]{virtual anchor}
\acrodef{dnr}[DNR]{dense-to-noise ratio}
\acrodef{pbo}[PBO]{potential bias object}
\acrodef{npbo}[NPBO]{new \ac{pbo}}
\acrodef{lpbo}[LPBO]{legacy \ac{pbo}}

